Improving Zero-Shot Event Extraction via Sentence Simplification

The success of sites such as ACLED and Our World in Data have demonstrated the massive utility of extracting events in structured formats from large volumes of textual data in the form of news, social media, blogs and discussion forums. Event extraction can provide a window into ongoing geopolitical crises and yield actionable intelligence. With the proliferation of large pretrained language models, Machine Reading Comprehension (MRC) has emerged as a new paradigm for event extraction in recent times. In this approach, event argument extraction is framed as an extractive question-answering task. One of the key advantages of the MRC-based approach is its ability to perform zero-shot extraction. However, the problem of long-range dependencies, i.e., large lexical distance between trigger and argument words and the difficulty of processing syntactically complex sentences plague MRC-based approaches. In this paper, we present a general approach to improve the performance of MRC-based event extraction by performing unsupervised sentence simplification guided by the MRC model itself. We evaluate our approach on the ICEWS geopolitical event extraction dataset, with specific attention to `Actor' and `Target' argument roles. We show how such context simplification can improve the performance of MRC-based event extraction by more than 5% for actor extraction and more than 10% for target extraction.

==> sections/evaluation.tex <==
\section{Evaluation}
During evaluation we are interested in the following research questions 1) - Can large pretrained language models finetuned for RC outperform traditional sequence labeling models for extraction? 2) - Does sentence simplification improve the performance of RC-based models? If yes, why?

\subsubsection{Datasets}
1) ICEWS - Actor / Target Extraction. Table ~\ref{tab:icews_predicates} gives an overview of the event predicates and the corresponding modified predicates that served as filtering keywords in our dataset which we then used to generate questions.
2) ACE - Event Trigger Extraction / Argument Extraction

1-Trigger Extraction - Identify the event type
2-Invoke questions for its argument roles
3-Evaluate for with/w/o unsupervised simplification.

\begin{table*}[]
\centering
\caption{This table lists the ICEWS event types used and their corresponding predicates that were identified for generating question templates.}
\label{tab:icews_predicates}
\begin{tabular}{ll}
\hline
Event Type                                   & Predicates                                                                                                                                             \\ \hline
Abduct, hijack, or take hostage             & kidnapped, abducting, abducted, captured                                                                                                                          \\
Accuse                                      & blame, blaming, accused, alleged, accusing                                                                                                                        \\
Apologize                                   & apologize, apology                                                                                                                                                \\
Assassinate                                 & carried out assassination of, assassinate                                                                                                                         \\
Bring lawsuit against                       & is suing someone, sued, has sued, filed a suit against                                                                                                            \\
Demonstrate or rally                        & condemn, protest, demonstrate                                                                                                                                     \\
Arrest, detain, or charge with legal action & \begin{tabular}[c]{@{}l@{}}arrested, sentenced, detained, nabbed, captured, arresting,\\  capture, jailed, routinely arrested, prosecuted, convicted\end{tabular} \\
Use conventional military force             & killed, shelled, combating, shells, strikes, strike, kill                                                                                                        
\end{tabular}
\end{table*}


\section{Experiments}
Following prior work in information extraction, we view event extraction as a span extraction task.
We compared our approach with a variety of span-based methods. We extracted the best span(s) and computed an exact match F1 score or a char-based F1 as previously used ~\cite{Seo2017BidirectionalAF} score matching against the ground truth answer.

\subsection{Datasets}
The first dataset we evaluate on is the ICEWS event dataset \footnote{https://dataverse.harvard.edu/dataverse/icews} from years 2013 to 2016. Event data consists of coded interactions between socio-political actors (i.e., cooperative or hostile actions between individuals, groups, sectors and nation states). Events are automatically identified and extracted from news articles by the BBN ACCENT event coder. These events are essentially triples consisting of a source actor, an event type (according to the CAMEO taxonomy of events), and a target actor. 

\subsection{Comparative Methods}

1. We implement a bi-lstm-crf ~\cite{huang2015bidirectional} baseline. This is essentially a bidirectional LSTM model followed by a CRF-layer ~\cite{crf}. We use the BIO labeling scheme for this task. We chose B-ACT, I-ACT and tags for tokens at the beginning and inside of an actor entity and B-TARG and I-TARG as tags tokens for at the beginning and inside of Target entities. We use the 'O' tags for any tokens outside of these entities. We used early stopping to prevent overfitting.


2. We use the TransformerQA ~\cite{NIPS2017_7181} model finetuned on Squad-v-0.1 and use the best span predicted as the answer

3. We finetuned BERT-base-uncased model on the ICEWS dataset to extract the most likely span from the text. 

4. We run BERT for token classification to extract sentences.

5. Next we apply the proposed sentence simplification approach to disambiguate the source context and run the baselines again.

6. In each case we visualize the attention weights to understand where the model puts emphasis during each baseline and how the weights change, changing the performance after simplification.

7. 



\section{Results}
We measure the performance of our models using two metrics exact-match F1 and a softer metric char-F1 as used in ~\citep{Seo2017BidirectionalAF}. 
 


% Please add the following required packages to your document preamble:
\begin{table*}[t!]
\begin{tabular}{@{}lll@{}}
\toprule
Model                                & Actor Exact F1 & Target Exact F1 \\ \midrule
bilstm-crf                           & 61.3      & 71.1       \\
Dygie++                              &       &        \\
Bert-QA (finetune Squad)                              &     &       \\
Bert-QA (finetune)                              &    76.3   &  84.5      \\
Bert-QA (finetune) + ClauseIE simplification             &       &        \\ 
Bert-QA(finetune) + simplification             &       &        \\ 
Bert-QA(finetune) + simplification + QA Reward &       &        \\
SpanBERT  &       &        \\
SpanBERT + simplification &       &        \\
\bottomrule
\end{tabular}
\end{table*}
